Dynamic Line Rating using Hyper-local Weather Predictions: A Machine Learning Approach

Dynamic Line Rating (DLR) systems are crucial for renewable energy integration in transmission networks. However, traditional methods relying on sensor data face challenges due to the impracticality of installing sensors on every pole or span. Additionally, sensor-based approaches may struggle predicting DLR in rapidly changing weather conditions. This paper proposes a novel approach, leveraging machine learning (ML) techniques alongside hyper-local weather forecast data. Unlike conventional methods, which solely rely on sensor data, this approach utilizes ML models trained to predict hyper-local weather parameters on a full network scale. Integrating topographical data enhances prediction accuracy by accounting for landscape features and obstacles around overhead lines. The paper introduces confidence intervals for DLR assessments to mitigate risks associated with uncertainties. A case study from Estonia demonstrates the practical implementation of the proposed methodology, highlighting its effectiveness in real-world scenarios. By addressing limitations of sensor-based approaches, this research contributes to the discourse of renewable energy integration in transmission systems, advancing efficiency and reliability in the power grid.

==> bibliography.tex <==
% Encoding: UTF-8
% https://www.doi2bib.org/ is helpful


@article{tu2022maxvit,
  title={MaxViT: Multi-Axis Vision Transformer},
  author={Tu, Zhengzhong and Talebi, Hossein and Zhang, Han and Yang, Feng and Milanfar, Peyman and Bovik, Alan and Li, Yinxiao},
  journal={ECCV},
  year={2022},
}

@article{cbam,
  author       = {Sanghyun Woo and
                  Jongchan Park and
                  Joon{-}Young Lee and
                  In So Kweon},
  title        = {{CBAM:} Convolutional Block Attention Module},
  journal      = {CoRR},
  volume       = {abs/1807.06521},
  year         = {2018},
  url          = {http://arxiv.org/abs/1807.06521},
  eprinttype    = {arXiv},
  eprint       = {1807.06521},
  timestamp    = {Mon, 13 Aug 2018 16:48:20 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1807-06521.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{arome,
author = {Seity, Yann and Brousseau, Pierre and Malardel, Sylvie and Hello, G. and Bénard, P. and Bouttier, F. and Lac, C. and Masson, Valéry},
year = {2011},
month = {03},
pages = {976-991},
title = {The AROME-France convective-scale operational model},
volume = {139},
journal = {Monthly Weather Review},
doi = {10.1175/2010MWR3425.1}
}

@misc{2015resnet,
      title={Deep Residual Learning for Image Recognition}, 
      author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
      year={2015},
      eprint={1512.03385},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@Article{Shahidehpour2005,
  author   = {Shahidehpour, M. and Ferrero, R.},
  journal  = {IEEE Power and Energy Magazine},
  title    = {Time management for assets: chronological strategies for power system asset management},
  year     = {2005},
  issn     = {1558-4216},
  month    = {May},
  number   = {3},
  pages    = {32-38},
  volume   = {3},
  abstract = {This paper discusses how the coordination of time scales for asset management plays a critical role in strategic decisions. It categorizes asset management based on possible time scales: real-time asset management; short-term asset management; midterm asset management; and long-term asset management. The paper asserts that the realization of chronological asset management in the field could lead to the better operation and management of power systems in a competitive era.},
  doi      = {10.1109/MPAE.2005.1436498},
}

@InProceedings{Mitsuhiro2020,
  author    = {Mitsuhiro, Nakamura and Shigeyuki, Tsukao and Masao, Nakai and Kouji, Miyashita},
  booktitle = {2020 International Symposium on Electrical Insulating Materials (ISEIM)},
  title     = {Approach to Asset Management of Substation Equipment in Japan},
  year      = {2020},
  month     = {Sep.},
  pages     = {68-71},
  abstract  = {IEC white paper “Strategic Asset management of Power Networks” was published in 2015, and TC123 “Management of network assets in power system” is working towards the IEC standardization since 2017. The environment surrounding Japanese utilities is changing, and the need for asset management is increasing. This paper describes the environment surrounding the electric power industry in Japan and the necessity of asset management. And this paper reports example of asset management for substation equipment (Transformers and circuit breakers) by Japanese utilities. First, the environment surrounding the electric power industry in Japan is summarized. The aging of equipment owned by utilities, the decrease in the number of electric power engineers due to the declining birthrate, and a decrease in demand for electric power are some of the problems facing us. Under these circumstances, it is not realistic to replace equipment based on aging due to cost, construction, and network operational constraints. Because many equipment need to be replaced in a short period. Therefore, in order to realize effective investment and equalization of the replacement amount, asset management based on the condition evaluation and evaluation of consequence is important. Next, this paper reports the case of asset management for substation equipment by some Japanese utilities. This paper describes asset management (such as “scoring”, “risk matrix” and other methods) for transformers and circuit breakers, in which condition evaluation of equipment (such as dissolved gas analysis results of transformers and the number of operations of circuit breakers) and evaluation of consequence (such as power system importance and environmental impacts) are evaluated. In addition, important evaluation items in each case are described.},
}

@article{solar_SHARMA1965183,
title = {Interrelationships between total, direct, and diffuse solar radiation in the tropics},
journal = {Solar Energy},
volume = {9},
number = {4},
pages = {183-192},
year = {1965},
issn = {0038-092X},
doi = {https://doi.org/10.1016/0038-092X(65)90045-9},
url = {https://www.sciencedirect.com/science/article/pii/0038092X65900459},
author = {M.R. Sharma and R.S. Pal},
abstract = {Formulas that directly yield intensities of direct and diffuse radiation on horizontal surfaces from measurements of hourly total radiation only have been developed. Alternatively, atmospheric turbidity and solar altitude can also yield similar results. These formulas result in obtaining relations similar to those given by Parmelee from data collected in the United States. The data for New Delhi have also been shown to agree with these correlations. Computed values of direct solar radiation on a horizontal surface or at normal incidence, are expressed by a mathematical expression that is shown to agree closely with the computed values obtained by Rao and Seshadri. Correlation between hourly direct and total transmission factors has been shown to depend on the solar altitude, in addition to the atmospheric turbidity.}
}

@article{pvlib, doi = {10.21105/joss.05994}, url = {https://doi.org/10.21105/joss.05994}, year = {2023}, publisher = {The Open Journal}, volume = {8}, number = {92}, pages = {5994}, author = {Kevin S. Anderson and Clifford W. Hansen and William F. Holmgren and Adam R. Jensen and Mark A. Mikofski and Anton Driesse}, title = {pvlib python: 2023 project update}, journal = {Journal of Open Source Software} }

@InProceedings{Suzuki2010,
  author    = {Suzuki, Yotaro and Kojima, Hiroki and Hayakawa, Naoki and Endo, Fumihiro and Okubo, Hitoshi},
  booktitle = {2010 IEEE International Symposium on Electrical Insulation},
  title     = {Optimization of asset management in high voltage substation based on equipment monitoring and power system operation},
  year      = {2010},
  month     = {June},
  pages     = {1-5},
  abstract  = {This paper presents a new optimization approach of maintenance strategy for equipment in a transmission and distribution (T&D) system. In this approach, a present and future equipment performance is estimated by using monitoring data, and impacts of performance in each equipment on a whole T&D system are evaluated. By minimizing the impacts, suitable maintenance procedures and timing are derived. This approach is applied to a circuit breaker (CB) in an electric network, and its significance and usefulness are presented.},
  doi       = {10.1109/ELINSL.2010.5549579},
  issn      = {1089-084X},
}



@Comment{jabref-meta: databaseType:bibtex;}


@article{Trondle2020,
  doi = {10.1016/j.joule.2020.07.018},
  url = {https://doi.org/10.1016/j.joule.2020.07.018},
  year = {2020},
  month = sep,
  publisher = {Elsevier {BV}},
  volume = {4},
  number = {9},
  pages = {1929--1948},
  author = {Tim Tr\"{o}ndle and Johan Lilliestam and Stefano Marelli and Stefan Pfenninger},
  title = {Trade-Offs between Geographic Scale,  Cost,  and Infrastructure Requirements for Fully Renewable Electricity in Europe},
  journal = {Joule}
}

@article{Child2019,
  doi = {10.1016/j.renene.2019.02.077},
  url = {https://doi.org/10.1016/j.renene.2019.02.077},
  year = {2019},
  month = aug,
  publisher = {Elsevier {BV}},
  volume = {139},
  pages = {80--101},
  author = {Michael Child and Claudia Kemfert and Dmitrii Bogdanov and Christian Breyer},
  title = {Flexible electricity generation,  grid exchange and storage for the transition to a 100{\%} renewable energy system in Europe},
  journal = {Renewable Energy}
}

@article{Joskow2020,
  doi = {10.1016/j.joule.2019.10.011},
  url = {https://doi.org/10.1016/j.joule.2019.10.011},
  year = {2020},
  month = jan,
  publisher = {Elsevier {BV}},
  volume = {4},
  number = {1},
  pages = {1--3},
  author = {Paul L. Joskow},
  title = {Transmission Capacity Expansion Is Needed to Decarbonize the Electricity Sector Efficiently},
  journal = {Joule}
}

@article{Lai2022,
  doi = {10.1016/j.egyr.2022.02.085},
  url = {https://doi.org/10.1016/j.egyr.2022.02.085},
  year = {2022},
  month = nov,
  publisher = {Elsevier {BV}},
  volume = {8},
  pages = {3263--3288},
  author = {Ching-Ming Lai and Jiashen Teh},
  title = {Comprehensive review of the dynamic thermal rating system for sustainable electrical power systems},
  journal = {Energy Reports}
}

@inproceedings{Molinar2019,
  doi = {10.1109/africon46755.2019.9134046},
  url = {https://doi.org/10.1109/africon46755.2019.9134046},
  year = {2019},
  month = sep,
  publisher = {{IEEE}},
  author = {Gabriela Molinar and Mengyu Li and Wilhelm Stork},
  title = {Positioning of distributed weather overhead line monitoring based on historical weather data},
  booktitle = {2019 {IEEE} {AFRICON}}
}

@article{Phillips2017,
  doi = {10.1016/j.renene.2017.02.072},
  url = {https://doi.org/10.1016/j.renene.2017.02.072},
  year = {2017},
  month = aug,
  publisher = {Elsevier {BV}},
  volume = {108},
  pages = {380--389},
  author = {Tyler Phillips and Rey DeLeon and Inanc Senocak},
  title = {Dynamic rating of overhead transmission lines over complex terrain using a large-eddy simulation paradigm},
  journal = {Renewable Energy}
}

@article{Seppa1993,
  doi = {10.1109/61.252680},
  url = {https://doi.org/10.1109/61.252680},
  year = {1993},
  month = jul,
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {8},
  number = {3},
  pages = {1536--1550},
  author = {T.O. Seppa},
  title = {A practical approach for increasing the thermal capabilities of transmission lines},
  journal = {{IEEE} Transactions on Power Delivery}
}

@book{Glover2012,
    author = {J Duncan Glover and Mulukutla S Sarma and Thomas J Overbye},
    title = {Power System Analysis And Design 5th Edition},
    publisher = {Cengage Learning},
    year = {2012}
}

@article{Karimi2018,
  doi = {10.1016/j.rser.2018.04.001},
  url = {https://doi.org/10.1016/j.rser.2018.04.001},
  year = {2018},
  month = aug,
  publisher = {Elsevier {BV}},
  volume = {91},
  pages = {600--612},
  author = {Soheila Karimi and Petr Musilek and Andrew M. Knight},
  title = {Dynamic thermal rating of transmission lines: A review},
  journal = {Renewable and Sustainable Energy Reviews}
}

@ARTICLE{Houseandtuttle,
  author={House, H. E. and Tuttle, P. D.},
  journal={Transactions of the American Institute of Electrical Engineers. Part III: Power Apparatus and Systems}, 
  title={Current-Carrying Capacity of ACSR}, 
  year={1958},
  volume={77},
  number={3},
  pages={1169-1173},
  keywords={Conductors;Testing;Temperature;Surface resistance;Steel;Wind speed;Aluminum;Laboratories;Equations;Copper},
  doi={10.1109/AIEEPAS.1958.4500119}}

@article{elevation_dlrZ2022107338,
title = {Application of Digital Elevation Models to wind estimation for dynamic line rating},
journal = {International Journal of Electrical Power and Energy Systems},
volume = {134},
pages = {107338},
year = {2022},
issn = {0142-0615},
doi = {https://doi.org/10.1016/j.ijepes.2021.107338},
url = {https://www.sciencedirect.com/science/article/pii/S0142061521005779},
author = {R. Minguez and R. Martinez and M. Manana and D. Cuasante and R. Garañeda},
keywords = {Dynamic Line Rating, Digital Elevation Model, Wind propagation, Effective wind, Renewable integration},
abstract = {The distribution of renewable energy is now a reality in power distribution grids. This type of energy demands a new and effective electrical infrastructure to manage its intermittency. A dynamic line rating system provides an alternative for new assets with a large capital investment. Dynamic line rating studies and projects have revealed several issues that need to be solved to create safe and accurate systems. One of the major challenges is finding the best monitoring point. Because the ampacity changes along the overhead line, the objective of this study was to develop a methodology to calculate the distributed ampacity along the line using digital elevation and wind propagation models. Finally, an example of this methodology was applied to two real distribution lines: a short line and long line. A comparison between the new methodology and the current operation methodologies found that the point with the least cooling along the line differed depending on the wind direction. Thus, the ampacity could be overestimated by the commonly used dynamic line rating systems. Moreover, the proposed Simulated Distributed Wind Estimation (SWDE) is an economical alternative to a distributed monitoring system.}
}

@ARTICLE{8269366,
  author={Bhattarai, Bishnu P. and Gentle, Jake P. and McJunkin, Timothy and Hill, Porter J. and Myers, Kurt S. and Abboud, Alexander W. and Renwick, Rodger and Hengst, David},
  journal={IEEE Transactions on Power Delivery}, 
  title={Improvement of Transmission Line Ampacity Utilization by Weather-Based Dynamic Line Rating}, 
  year={2018},
  volume={33},
  number={4},
  pages={1853-1863},
  keywords={Wind speed;Conductors;Power system dynamics;Electric potential;Glass;Dynamic line rating (DLR);general line ampacity state solver;grid integration;power system planning},
  doi={10.1109/TPWRD.2018.2798411}}


@article{Matus2012,
  doi = {10.1109/tpwrd.2012.2185254},
  url = {https://doi.org/10.1109/tpwrd.2012.2185254},
  year = {2012},
  month = apr,
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {27},
  number = {2},
  pages = {1002--1009},
  author = {Marcelo Matus and Doris Saez and Mark Favley and Carlos Suazo-Martinez and Jos{\'{e}} Moya and Guillermo Jimenez-Estevez and Rodrigo Palma-Behnke and Gabriel Olguin and Pablo Jorquera},
  title = {Identification of Critical Spans for Monitoring Systems in Dynamic Thermal Rating},
  journal = {{IEEE} Transactions on Power Delivery}
}

@techreport{Oncor2013,
    author = {Justin Johnson and Cale Smith and Mike Young and Ken Donohoo and Ross Owen and Eddit Clark},
    title = {Dynamic Line Rating Oncor Electric Delivery Smart Grid Program},
    institution = {University of North Texas Libraries},
    year = {2013} 
}

@techreport{IRENA2020,
    author = {IRENA},
    title = {Innovation landscape brief: Dynamic line rating},
    institution = {International Renewable Energy Agency},
    year = {2020} 
}

@article{Glaum2023,
  doi = {10.1016/j.apenergy.2023.121199},
  url = {https://doi.org/10.1016/j.apenergy.2023.121199},
  year = {2023},
  month = aug,
  publisher = {Elsevier {BV}},
  volume = {343},
  pages = {121199},
  author = {Philipp Glaum and Fabian Hofmann},
  title = {Leveraging the existing German transmission grid with dynamic line rating},
  journal = {Applied Energy}
}

@techreport{Cigre601,
    author = {CIGRE},
    title = {{TB601:} GUIDE FOR THERMAL RATING CALCULATIONS OF OVERHEAD LINES},
    institution = {CIGRE},
    year = {2014} 
}

@article{wind_speed_and_preiciton_analysis,
title = {A joint probability density function of wind speed and direction for wind energy analysis},
journal = {Energy Conversion and Management},
volume = {49},
number = {6},
pages = {1309-1320},
year = {2008},
issn = {0196-8904},
doi = {https://doi.org/10.1016/j.enconman.2008.01.010},
url = {https://www.sciencedirect.com/science/article/pii/S0196890408000228},
author = {José A. Carta and Penélope Ramírez and Celia Bueno},
keywords = {Circular–linear distributions, Wind direction probability distributions, Wind speed probability distributions, Wind rose, Wind power density, Wind turbine energy output},
abstract = {A very flexible joint probability density function of wind speed and direction is presented in this paper for use in wind energy analysis. A method that enables angular–linear distributions to be obtained with specified marginal distributions has been used for this purpose. For the marginal distribution of wind speed we use a singly truncated from below Normal–Weibull mixture distribution. The marginal distribution of wind direction comprises a finite mixture of von Mises distributions. The proposed model is applied in this paper to wind direction and wind speed hourly data recorded at several weather stations located in the Canary Islands (Spain). The suitability of the distributions is judged from the coefficient of determination R2. The conclusions reached are that the joint distribution proposed in this paper: (a) can represent unimodal, bimodal and bitangential wind speed frequency distributions, (b) takes into account the frequency of null winds, (c) represents the wind direction regimes in zones with several modes or prevailing wind directions, (d) takes into account the correlation between wind speeds and its directions. It can therefore be used in several tasks involved in the evaluation process of the wind resources available at a potential site. We also conclude that, in the case of the Canary Islands, the proposed model provides better fits in all the cases analysed than those obtained with the models used in the specialised literature on wind energy.}
}

@techreport{EU_Commission_RE_Directive_2021,
    author = {European Commission},
    title = {Commission presents Renewable Energy Directive revision},
    institution = {European Commission},
    year = {2021} 
}



@Article{wind_speed_and_direction_pdf,
AUTHOR = {Feng, Ju and Shen, Wen Zhong},
TITLE = {Modelling Wind for Wind Farm Layout Optimization Using Joint Distribution of Wind Speed and Wind Direction},
JOURNAL = {Energies},
VOLUME = {8},
YEAR = {2015},
NUMBER = {4},
PAGES = {3075--3092},
URL = {https://www.mdpi.com/1996-1073/8/4/3075},
ISSN = {1996-1073},
ABSTRACT = {Reliable wind modelling is of crucial importance for wind farm development. The common practice of using sector-wise Weibull distributions has been found inappropriate for wind farm layout optimization. In this study, we propose a simple and easily implementable method to construct joint distributions of wind speed and wind direction, which is based on the parameters of sector-wise Weibull distributions and interpolations between direction sectors. It is applied to the wind measurement data at Horns Rev and three different joint distributions are obtained, which all fit the measurement data quite well in terms of the coefficient of determination . Then, the best of these joint distributions is used in the layout optimization of the Horns Rev 1 wind farm and the choice of bin sizes for wind speed and wind direction is also investigated. It is found that the choice of bin size for wind direction is especially critical for layout optimization and the recommended choice of bin sizes for wind speed and wind direction is finally presented.},
DOI = {10.3390/en8043075}
}





@article{lognormal_Baran_2015,
   title={Log‐normal distribution based Ensemble Model Output Statistics models for probabilistic wind‐speed forecasting},
   volume={141},
   ISSN={1477-870X},
   url={http://dx.doi.org/10.1002/qj.2521},
   DOI={10.1002/qj.2521},
   number={691},
   journal={Quarterly Journal of the Royal Meteorological Society},
   publisher={Wiley},
   author={Baran, Sándor and Lerch, Sebastian},
   year={2015},
   month=mar, pages={2289–2299} }


@techreport{Cigre324,
    author = {CIGRE},
    title = {{TB324:} Sag-Tension calculation methods for overhead lines},
    institution = {CIGRE},
    year = {2016} 
}

@techreport{Cigre207,
    author = {CIGRE},
    title = {{TB207:} Thermal behaviour of overhead conductors},
    institution = {CIGRE},
    year = {2002} 
}

@techreport{Cigre299,
    author = {CIGRE},
    title = {{TB299:} Guide for the selection of weather parameters for bare overhead conductor ratings},
    institution = {CIGRE},
    year = {2006} 
}


@ARTICLE{IEEE738,
  author={IEEE},
  journal={IEEE Std 738-2012 (Revision of IEEE Std 738-2006 - Incorporates IEEE Std 738-2012 Cor 1-2013)}, 
  title={IEEE Standard for Calculating the Current-Temperature Relationship of Bare Overhead Conductors}, 
  year={2013},
  volume={},
  number={},
  pages={1-72},
  keywords={IEEE standards;Temperature measurement;Power transmission lines;Measurement;bare overhead lines;current-temperature relationship;IEEE 738(TM)},
  doi={10.1109/IEEESTD.2013.6692858}}
}

@inbook{ECMWF-IFS,
  author = {ECMWF},
  title = {IFS Documentation CY48R1 - Part III: Dynamics and Numerical Procedures},
  abstract = {<p>Chapter 1 Introduction<br />
Chapter 2 Basic equations and discretisation<br />
Chapter 3 Semi-Lagrangian formulation</p>
},
  year = {2023},
  journal = {IFS Documentation CY48R1},
  number = {3},
  month = {06/2023},
  publisher = {ECMWF},
  doi = {10.21957/26f0ad3473},
}
@article{CDF_wind_turbine,
author = {Hattori, Yasuo and Tanaka, Nobukazu and Moeng, Chin-Hoh and Suto, Hitoshi and Ishihara, Shuji and Eguchi, Yuzuru and Hirakuchi, Hiromaru and Sugimoto, Soichiro},
year = {2011},
month = {04},
pages = {342-356},
title = {Numerical Simulation of Atmospheric Turbulence for Assessment of Wind Turbine},
volume = {6},
journal = {Journal of Fluid Science and Technology},
doi = {10.1299/jfst.6.342}
}

@article{DLr_forecasting,
author = {Douglass, Dale and Nguyen, Minh and Jardini, J.A. and Gentle, Jake and Chen, Hong and Goodwin, Tip and Chisholm, William and Grant, Ian and Nuthalapati, Sarma and Davis, Cody and Traynor, Paula and Xu, Charles and Hurst, Neil and Kluge, Robert},
year = {2019},
month = {07},
pages = {1-1},
title = {A Review of Dynamic Thermal Line Rating Methods With Forecasting},
volume = {PP},
journal = {IEEE Transactions on Power Delivery},
doi = {10.1109/TPWRD.2019.2932054}
}

@article{Forecast_dlr_MICHIORRI20151713,
title = {Forecasting for dynamic line rating},
journal = {Renewable and Sustainable Energy Reviews},
volume = {52},
pages = {1713-1730},
year = {2015},
issn = {1364-0321},
doi = {https://doi.org/10.1016/j.rser.2015.07.134},
url = {https://www.sciencedirect.com/science/article/pii/S1364032115007819},
author = {Andrea Michiorri and Huu-Minh Nguyen and Stefano Alessandrini and John Bjørnar Bremnes and Silke Dierer and Enrico Ferrero and Bjørn-Egil Nygaard and Pierre Pinson and Nikolaos Thomaidis and Sanna Uski},
keywords = {Rating, Overhead lines, Forecast, Smart grid},
abstract = {This paper presents an overview of the state of the art on the research on Dynamic Line Rating forecasting. It is directed at researchers and decision-makers in the renewable energy and smart grids domain, and in particular at members of both the power system and meteorological community. Its aim is to explain the details of one aspect of the complex interconnection between the environment and power systems. The ampacity of a conductor is defined as the maximum constant current which will meet the design, security and safety criteria of a particular line on which the conductor is used. Dynamic Line Rating (DLR) is a technology used to dynamically increase the ampacity of electric overhead transmission lines. It is based on the observation that the ampacity of an overhead line is determined by its ability to dissipate into the environment the heat produced by Joule effect. This in turn is dependent on environmental conditions such as the value of ambient temperature, solar radiation, and wind speed and direction. Currently, conservative static seasonal estimations of meteorological values are used to determine ampacity. In a DLR framework, the ampacity is estimated in real time or quasi-real time using sensors on the line that measure conductor temperature, tension, sag or environmental parameters such as wind speed and air temperature. Because of the conservative assumptions used to calculate static seasonal ampacity limits and the variability of weather parameters, DLRs are considerably higher than static seasonal ratings. The latent transmission capacity made available by DLRs means the operation time of equipment can be extended, especially in the current power system scenario, where power injections from Intermittent Renewable Sources (IRS) put stress on the existing infrastructure. DLR can represent a solution for accommodating higher renewable production whilst minimizing or postponing network reinforcements. On the other hand, the variability of DLR with respect to static seasonal ratings makes it particularly difficult to exploit, which explains the slow take-up rate of this technology. In order to facilitate the integration of DLR into power system operations, research has been launched into DLR forecasting, following a similar avenue to IRS production forecasting, i.e. based on a mix of statistical methods and meteorological forecasts. The development of reliable DLR forecasts will no doubt be seen as a necessary step for integrating DLR into power system management and reaping the expected benefits.}
}

@article{CDF_NAKAO2019103970,
title = {Reconciliation of computational fluid dynamics and observations in complex terrain through conditional resampling},
journal = {Journal of Wind Engineering and Industrial Aerodynamics},
volume = {195},
pages = {103970},
year = {2019},
issn = {0167-6105},
doi = {https://doi.org/10.1016/j.jweia.2019.103970},
url = {https://www.sciencedirect.com/science/article/pii/S0167610519305707},
author = {Keisuke Nakao and Yasuo Hattori},
keywords = {Large-eddy simulation, Complex terrain, Turbulence statistics}
}

@article{Dickinson_Errico_Giorgi_Bates_1989, title={A regional climate model for the Western United States}, volume={15}, DOI={10.1007/bf00240465}, number={3}, journal={Climatic Change}, author={Dickinson, RobertE. and Errico, RonaldM. and Giorgi, Filippo and Bates, GaryT.}, year={1989}} 

@Article{stat-downscaling,
AUTHOR = {Tabari, H. and Paz, S. M. and Buekenhout, D. and Willems, P.},
TITLE = {Comparison of statistical downscaling methods for climate change impact analysis on precipitation-driven drought},
JOURNAL = {Hydrology and Earth System Sciences},
VOLUME = {25},
YEAR = {2021},
NUMBER = {6},
PAGES = {3493--3517},
URL = {https://hess.copernicus.org/articles/25/3493/2021/},
DOI = {10.5194/hess-25-3493-2021}
}

@article{bayesian-nnet,
  author       = {Vikram Mullachery and
                  Aniruddh Khera and
                  Amir Husain},
  title        = {Bayesian Neural Networks},
  journal      = {CoRR},
  volume       = {abs/1801.07710},
  year         = {2018},
  url          = {http://arxiv.org/abs/1801.07710},
  eprinttype    = {arXiv},
  eprint       = {1801.07710},
  timestamp    = {Mon, 13 Aug 2018 16:48:31 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1801-07710.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@article{vision-transformers,
  author       = {Niki Parmar and
                  Ashish Vaswani and
                  Jakob Uszkoreit and
                  Lukasz Kaiser and
                  Noam Shazeer and
                  Alexander Ku},
  title        = {Image Transformer},
  journal      = {CoRR},
  volume       = {abs/1802.05751},
  year         = {2018},
  url          = {http://arxiv.org/abs/1802.05751},
  eprinttype    = {arXiv},
  eprint       = {1802.05751},
  timestamp    = {Mon, 13 Aug 2018 16:48:00 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1802-05751.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@techreport{osti_1895360,
title = {Forecasting Dynamic Line Rating with Spatial Variation Considerations},
author = {Phillips, Tyler Bennett and Abboud, Alexander W and Starks, Brandon Edward and Lehmer, Jacob P and Gentle, Jake P},
abstractNote = {Dynamic line rating (DLR) is a technology that allows the ampacity of an electrical conductor to be calculated using real-time or forecasted weather conditions. Historically, the ampacity of a conductor has been determined using a static line rating method which assumes conservative weather assumptions. Therefore, not only can DLR give a more accurate measurement of the true ampacity of a conductor, but it can also increase its ampacity during weather conditions with greater thermal mitigations. The two primary cooling factors in the ampacity calculations are wind speed and direction. In complex terrain, wind speed and direction can have large variations over short distances. Therefore, accurately identifying the limiting span of a transmission line requires high spatial resolution of the wind along its path. One solution is to install dense weather stations along their path, though this can become costly over long distances. Therefore, researchers have investigated the use of Computation Fluid Dynamic (CFD) simulations to accurately compute the wind field along the path of a transmission line and use these results to identify the limiting section of the conductor. This work presents a case study that evaluates the coupling of CFD simulations and forecasted weather simulations using the High-Resolution Rapid Refresh (HRRR) model points over a 2-year span within a region in south eastern Idaho. The primary goal of the work is the evaluation of the number of HRRR model points used, i.e., weather stations, along the path of the line and the accuracy of the resulting DLR ampacity. This was done using 4, 10, 17, 26, and 35 HRRR model points along two transmission line paths. The results indicate that as the number of model points are increased, the DLR ampacity of the lines decrease, yet converge as more points are added and demonstrate little change with additional HRRR points. It is expected that these results can help transmission line operators identify the number of weather stations that must be installed when coupled with CFD simulations and DLR ampacity to ensure accurate ratings and safe operations.},
url = {https://www.osti.gov/biblio/1895360}, 
place = {United States},
institution = {Idaho National Laboratory},
year = {2021},
month = {12}
}

@misc{OpenStreetMap,
   author = {{OpenStreetMap contributors}},
   title = {{Planet dump retrieved from https://planet.osm.org }},
   howpublished = "\url{ https://www.openstreetmap.org }",
   year = {2017},
 }

 @misc{Estonian_Land_Board,
   author = {{Estonian Land Board}},
   title = {{Elevation data: Estonian Land Board 2023}},
   howpublished = "\url{ https://geoportaal.maaamet.ee/eng/Maps-and-Data/Elevation-data/Download-Elevation-Data-p664.html}",
   year = {2023},
 }

 @misc{metno,
   author = {{Norwegian Meteorological Institute }},
   title = {{Norwegian Meteorological Institute }},
   howpublished = "\url{ http://met.no/)). }",
   year = {2024},
 }

@article{KANG2020102086,
title = {Computational fluid dynamics simulation of tree effects on pedestrian wind comfort in an urban area},
journal = {Sustainable Cities and Society},
volume = {56},
pages = {102086},
year = {2020},
issn = {2210-6707},
doi = {https://doi.org/10.1016/j.scs.2020.102086},
url = {https://www.sciencedirect.com/science/article/pii/S2210670720300731},
author = {Geon Kang and Jae-Jin Kim and Wonsik Choi},
keywords = {Beaufort wind-force scale, CFD model, Pedestrian wind comfort, Tree drag parameterization, Urban area},
abstract = {In this study, we applied a computational fluid dynamics (CFD) model incorporating a tree drag parameterization scheme to investigate how the presence of trees improved pedestrian wind comfort on the urban campus of Pukyong National University (PKNU). We comprehensively analyzed pedestrian wind comfort considering wind inflow direction and observed frequency. To validate the CFD model, we conducted sensitivity simulations by varying the vertical profiles of leaf area density (LAD) and compared our CFD simulations with previous field measurements and simulation results. The adjusted LAD profile yielded the best reproduction of measured wind speeds and turbulent kinetic energy behind trees, demonstrating performance similar to that of a large-eddy simulation (LES) model. We applied the CFD model to investigate the effect of trees on pedestrian wind comfort on the PKNU campus. Trees markedly improved pedestrian wind comfort when horizontally incoming airflow passed through the trees; however, there was little improvement in pedestrian wind comfort in regions where airflow rapidly descended the walls of tall buildings.}
}

==> graphs/flowchart.tex <==
\begin{tikzpicture}[node distance=0.4cm and 1.3cm, auto]
    % Define block styles
    \tikzstyle{block} = [rectangle, draw, fill=blue!20, text width=5em, text centered, rounded corners, minimum height=2.5em, font=\footnotesize]
    \tikzstyle{data} = [rectangle, draw, fill=green!20, text width=5em, text centered, rounded corners, minimum height=2.5em, font=\footnotesize]
    \tikzstyle{iteration} = [rectangle, draw, fill=blue!20, text width=5em, text centered, rounded corners, minimum height=2.5em, font=\footnotesize]
    \tikzstyle{start} = [rectangle, draw, fill=red!20, text width=5em, text centered, rounded corners, minimum height=2.5em, font=\bfseries\footnotesize]
    \tikzstyle{line} = [draw, -latex']
    \tikzstyle{line_dashed} = [draw, dashed, -latex']
    
    % Nodes
    \node [start] (start) {Start};
    \node [iteration, right=of start] (time) {Iterate Time Periods};
    \node [iteration, below=of time] (span) {Iterate Spans};
    \node [block, below=of span] (calculate) {Hyper-local Weather Prediction};
    \node [block, below= of calculate] (ci) {Confidence Intervals};
    \node [data, right=of calculate] (weather) {NWP};
    \node [data, left=of calculate] (terrain) {DTM and DSM};
    \node [data, right=of span] (parameters) {Conductor Parameters};
    \node [data, left=of span] (temp) {Allowed Span Temperatures};
    \node [block, below= of ci] (dlr) {DLR Calculation};
    \node [iteration, below=of dlr] (endspan) {Next Span Iteration};
    \node [iteration, below=of endspan] (endtime) {Next Time Period};
    \node [block, right=of dlr] (store) {Store DLR};
    \node [block, below=of store] (min) {Data Aggregation};

    \node [start, below=of min] (done) {End};
    
  
    % Arrows
    \path [line] (start) -- (time);
    \path [line] (time) -- (span);
    \path [line] (parameters) -- (span);
    \path [line] (temp) -- (span);
    \path [line] (span) -- (calculate);
    \path [line] (ci) -- (dlr);
    \path [line] (calculate) -- (ci);
    \path [line] (dlr) -- (endspan);
    \path [line] (dlr) -- (store);
    \path [line] (store) -- (min);
    \path [line] (min) -- (done);
    \path [line] (endspan) -- (endtime);
    \path [line] (weather) -- (calculate);
    \path [line] (terrain) -- (calculate);
    \path [line_dashed] (endspan.west) -- ++(-1,0)  -| ([xshift=-1cm]span.west) -- (span.west);
    \path [line_dashed] (endtime.east) -- ++(1,0)  -| ([xshift=1cm]time.east) -- (time.east);
\end{tikzpicture}
